DeepPCR: Parallelizing Sequential Operations in Neural Networks

Parallelization techniques have become ubiquitous for accelerating inference and training of deep neural networks. Despite this, several operations are still performed in a sequential manner. For instance, the forward and backward passes are executed layer-by-layer, and the output of diffusion models is produced by applying a sequence of denoising steps. This sequential approach results in a computational cost proportional to the number of steps involved, presenting a potential bottleneck as the number of steps increases. In this work, we introduce DeepPCR, a novel algorithm which parallelizes typically sequential operations in order to speed up inference and training of neural networks. DeepPCR is based on interpreting a sequence of $L$ steps as the solution of a specific system of equations, which we recover using the Parallel Cyclic Reduction algorithm. This reduces the complexity of computing the sequential operations from $\mathcal{O}(L)$ to $\mathcal{O}(\log_2L)$, thus yielding a speedup for large $L$. To verify the theoretical lower complexity of the algorithm, and to identify regimes for speedup, we test the effectiveness of DeepPCR in parallelizing the forward and backward pass in multi-layer perceptrons, and reach speedups of up to $30\times$ for the forward and $200\times$ for the backward pass. We additionally showcase the flexibility of DeepPCR by parallelizing training of ResNets with as many as 1024 layers, and generation in diffusion models, enabling up to $7\times$ faster training and $11\times$ faster generation, respectively, when compared to the sequential approach.

==> tikz_figs/latent_diffusion_speedup.tex <==
\pgfplotsset{
  newtonItsStyle/.style={
  	tick label style={font=\normalsize},
    ymin = 0.01, ymax = 20,
    ymajorgrids= true,
    unbounded coords=jump,
    xlabel= Latent Dimension,
    axis background/.style={fill=gray!10},
    legend style={at={(1.05,0.5)},anchor=west, font=\normalsize},
    % legend pos = outer north east,
    % cycle list = {{YlGnBu-D},{YlGnBu-E},{YlGnBu-F},{YlGnBu-G},{YlGnBu-H},{YlGnBu-J},{YlGnBu-L}},
    cycle list = {{YlGnBu-H},{YlGnBu-J},{YlGnBu-L}},
    clip=false
  }
}
\pgfplotsset{
  lineStyle/.style={
    line width=0.5mm,
    mark=*,
    mark options={solid},
    mark size=1pt
  }
}

\begin{figure}[tb!]
\vskip 0.0in
\centering
\resizebox{0.7\textwidth}{!}{
  \begin{tikzpicture}

    \begin{axis}[name=ax1, newtonItsStyle, title=Latent Diffusion Speedup, ylabel=Speedup, clip=true, ymin = 0, ymax = 12, xmin=0, xmax = 140]   
        \addlegendimage{empty legend}
        \addplot+[lineStyle, color={YlGnBu-H}] table[x index=0, y index=1, col sep=comma]{data/latent_diffusion_speedup.csv};
        \addlegendentry{{$steps=256$}};
        \addplot+[lineStyle, color={YlGnBu-J}] table[x index=0, y index=2, col sep=comma]{data/latent_diffusion_speedup.csv};
        \addlegendentry{{$steps=512$}};
        \addplot+[lineStyle, color={YlGnBu-L}] table[x index=0, y index=3, col sep=comma]{data/latent_diffusion_speedup.csv};
        \addlegendentry{{$steps=1024$}};
        \addplot[lineStyle, dotted, mark=none, color=black] coordinates {(0,1) (140,1)};
        \node[anchor=south west ] at (axis cs: 0,1.0) {$\text{speedup}=1$};
    \end{axis}

  \end{tikzpicture}}
\caption{\textit{Conditional Latent Diffusion.} Measured speedup for various latent diffusion models, as a function of the latent dimension. The speedup is more evident for large number of denoising steps. However, as we increase the latent dimension, the speedup is affected by collateral hardware and software issues as also observed in \Cref{sec::results::single}.}
\label{fig::speedup_latent_diffusion}
\vskip -0.2in
\end{figure}

